GALIC: Hybrid Multi-Qubitwise Pauli Grouping for Quantum Computing Measurement

Observable estimation is a core primitive in NISQ-era algorithms targeting quantum chemistry applications. To reduce the state preparation overhead required for accurate estimation, recent works have proposed various simultaneous measurement schemes to lower estimator variance. Two primary grouping schemes have been proposed: fully commutativity (FC) and qubit-wise commutativity (QWC), with no compelling means of interpolation. In this work we propose a generalized framework for designing and analyzing context-aware hybrid FC/QWC commutativity relations. We use our framework to propose a noise-and-connectivity aware grouping strategy: Generalized backend-Aware pauLI Commutation (GALIC). We demonstrate how GALIC interpolates between FC and QWC, maintaining estimator accuracy in Hamiltonian estimation while lowering variance by an average of 20\% compared to QWC. We also explore the design space of near-term quantum devices using the GALIC framework, specifically comparing device noise levels and connectivity. We find that error suppression has a more than $10\times$ larger impact on device-aware estimator variance than qubit connectivity with even larger correlation differences in estimator biases.

==> related_work.tex <==
\section{Related Works}
\paragraph{Grouped Simultaneous Measurement}
% Start off with simultaneous measurement schemes (QWC, FC) and the initial graph theoretic partitioning algorithms (e.g. Izmaylov minimum clique cover, Gokhale, Crawford)
Simultaneous measurement by Pauli grouping is one of the most widely-utilized measurement optimization schemes in production QC software packages~\cite{qiskit2024,mcclean_openfermion_2019,kottmann_tequila_2021}. While most packages use QWC grouping as the default behavior~\cite{qiskit2024,mcclean_openfermion_2019,kottmann_tequila_2021} for hardware efficiency, proposals for entanglement-based measurement schemes have been growing in popularity since 2019~\cite{gokhale_optimization_2020,gokhale2020n,crawford_efficient_2021,hamamura_efficient_2020}. Initial works focused largely on combinatorial optimization algorithms for constructing commuting groups, with a particular emphasis on solving NP-Hard Minimum Clique Cover reductions using heuristic methods~\cite{verteletskyi_measurement_2020,gokhale_optimization_2020,gokhale2020n,crawford_efficient_2021}. 
More recent efforts have focused on augmenting grouping schemes for lower variance estimation: including adaptive estimations of variance~\cite{wu_overlapped_2023,yen_deterministic_2023,shlosberg_adaptive_2023}, overlapping commuting groups~\cite{wu_overlapped_2023,yen_deterministic_2023}, canceling variance contribution with additional commuting operators~\cite{choi_improving_2022}, and iterative grouping/shot allocation algorithms using gradient-based methods~\cite{yen_deterministic_2023, shlosberg_adaptive_2023}. However, the aforementioned works either used QWC or FC commuting schemes. As such, their optimizations are orthogonal to GALIC, and can be naturally used with our grouping function. Notable exceptions are recent ``hardware-efficient commutativity'' (HEC) proposals from Refs.~\cite{escudero_hardware-efficient_2023,miller2022hardware}. We introduce HEC in Sec.~\ref{sec:topology_grouping} to demonstrate how our context-aware grouping functions naturally encapsulates existing proposals, and we compare HEC with our noise and topology aware proposal, GALIC, in Sec.~\ref{sec:eval}.

\paragraph{Classical Shadow Tomography}
Grouping is far from the only proposal for expectation value calculation via simultaneous measurement. Tomographic techniques such as Classical Shadows~\cite{huang_predicting_2020} have also been an area of focus for researchers in recent works. Quantum state tomography attempts to reconstruct quantum states by repeated measurement by sampling the trial state with randomized~\cite{huang_predicting_2020,hu_classical_2021,koh_classical_2022,hillmich_decision_2021,elben_randomized_2022} or derandomized~\cite{nakaji_measurement_2023, huang_efficient_2021} classically invertible measurement circuits. Recent works removing noisy estimator bias~\cite{koh_classical_2022}, improving computational scalability using matrix product state simulation~\cite{akhtar_scalable_2023}, and accounting for experimental error via semi-definite programming~\cite{cattaneo_self-consistent_2023} have all made classical shadows a viable option for simultaneous measurement.

Wu et al. 2023~\cite{wu_overlapped_2023} introduced a framework unifying grouping with tomographic techniques, proposing the ``Overlapping Grouped Measurement'' (OGM) scheme. Their efforts in generalizing and unifying measurement schemes are complementary to ours. The grouping function framework proposed here is entirely compatible with the formulations used by Wu and colleagues, as generalized grouping functions simply provide another tool for constructing the sets of Pauli bases used in their estimator construction.

% Next discuss recent efforts to improve performance by introducing overlapping groups, ghost paulis, iterative methods, etc (Izmaylov-heavy, need to find some other sources too). Add part about HEC, discuss their initial proposals


% Wrap up by discussing alternatives, namely tomographic techniques (Huang et al and derivative works) and their unification with SM in Wu et al. Explicitly reference Izmaylov's work showing overlapped SM outperforming tomography. 

 

% Mention Wang et al's Engineered Likely
\paragraph{Shot Overhead Optimization}
% Start off with the basic Lagrangian techniques discussed here, then move into the more advanced schemes using coefficient splitting, etc.
Our work focuses on measurement optimization via simultaneous measurement. Several recent works have also examined optimizations in shot allocation~\cite{gu_adaptive_2021,yen_deterministic_2023,zhu_optimizing_2024,gresch_guaranteed_2023}, improving on the straightforward Lagrangian methods used in Appendix~\ref{appdx:shot_lagrange}. Most are adaptive schemes which allocate shots depending on measurement statistics, either operator variance~\cite{yen_deterministic_2023, zhu_optimizing_2024} or estimated cost function gradients~\cite{gu_adaptive_2021}. 
Other works have proposed lowered measurement overhead by modifying the target Hamiltonian~\cite{zhao_measurement_2020, ralli_unitary_2023} and using ``engineered likelihood functions'' to produce lower-variance Bayesian estimators~\cite{wang_minimizing_2021}. 
% \subsection{QPU Design Analyses}

